A Unified Framework for Oscillatory Integral Transform: When to use NUFFT or Butterfly Factorization?

This paper concerns the fast evaluation of the matvec $g=Kf$ for $K\in \mathbb{C}^{N\times N}$, which is the discretization of the oscillatory integral transform $g(x) = \int K(x,\xi) f(\xi)d\xi$ with a kernel function $K(x,\xi)=\alpha(x,\xi)e^{2\pi\i \Phi(x,\xi)}$, where $\alpha(x,\xi)$ is a smooth amplitude function, and $\Phi(x,\xi)$ is a piecewise smooth phase function with $O(1)$ discontinuous points in $x$ and $\xi$. A unified framework is proposed to compute $Kf$ with $O(N\log N)$ time and memory complexity via the non-uniform fast Fourier transform (NUFFT) or the butterfly factorization (BF), together with an $O(N)$ fast algorithm to determine whether NUFFT or BF is more suitable. This framework works for two cases: 1) explicit formulas for the amplitude and phase functions are known, 2) only indirect access of the amplitude and phase functions are available. Especially in the case of indirect access, our main contributions are: 1) an $O(N\log N)$ algorithm for recovering the amplitude and phase functions is proposed based on a new low-rank matrix recovery algorithm, 2) a new stable and nearly optimal BF with amplitude and phase functions in a form of a low-rank factorization (IBF-MAT) is proposed to evaluate the matvec $Kf$. Numerical results are provided to demonstrate the effectiveness of the proposed framework.

==> figure/fig-MLF.tex <==
\begin{figure}[htp]
\begin{minipage}{\textwidth}
\centering
\resizebox{5.5cm}{!}{
\input{figure/fig-comp-modules/fig-M2}
}
$\approx$
\resizebox{1.5cm}{!}{
\input{figure/fig-comp-modules/fig-D2}
}
\resizebox{1.5cm}{!}{
\input{figure/fig-comp-modules/fig-M2}
}
\resizebox{5.5cm}{!}{
\input{figure/fig-comp-modules/fig-D3}
}\\
\end{minipage}
\caption{The middle level factorization of
    a $64\times 64$ matrix ${M}^2\approx C^2\bar{M}^2(R^2)^*$
    assuming $r_0=1$ and $r_\eps=4$.
    Grey blocks indicate nonzero blocks.
    $C^2$ and $R^2$ are block-diagonal matrices with $16$ blocks of size $4 \times 1$.
    The diagonal blocks of $C^2$ and $R^2$ are assembled
    according to Equation \eqref{eq:expression-C} and \eqref{eq:expression-R}, respectively, 
    as indicated by black rectangles.
    $\bar{M}^2$ is a $4\times 4$ block matrix with each block
    $\bar{M}^2_{i,j}$ itself an $4\times 4$ block matrix
    containing diagonal weights matrix on the $(j,i)$ block.}
\label{fig:compression-1D}
\end{figure}


==> figure/fig-SPMC.tex <==
\begin{figure}[htp]
\begin{minipage}{\textwidth}
\centering
\resizebox{4cm}{!}{
\input{figure/fig-comp-modules/fig-S}
}
\resizebox{1.5cm}{!}{
\input{figure/fig-comp-modules/fig-D}
}
=
\resizebox{1.5cm}{!}{
\input{figure/fig-comp-modules/fig-P}
}
$\approx$
\resizebox{1.5cm}{!}{
\input{figure/fig-comp-modules/fig-D}
}
\resizebox{1cm}{!}{
\input{figure/fig-comp-modules/fig-S2}
}\\
\end{minipage}
\caption{The structure-preserving matrix compression of type $(4,4,4,1)$ $SD=P\approx \tilde{D}\tilde{S}$, where $S\in \mathbb{C}^{16\times 16}$ (left matrix), $P\in \mathbb{C}^{16\times 4}$ (middle matrix), and $\tilde{S}\in \mathbb{C}^{4\times 4}$ (right matrix) are $4\times 4$ block matrices with the same sparsity pattern, $D\in \mathbb{C}^{16\times 4}$ (middle left matrix) and $\tilde{D}\in \mathbb{C}^{16\times 4}$ (middle right matrix) are $4\times 4$ block-diagonal matrices, }
\label{fig:SPMC}
\end{figure}


==> figure/fig-comp-modules/fig-K.tex <==
\begin{tikzpicture}[baseline=-0.5ex]
      \tikzset{every left delimiter/.style={xshift=-1ex},every right delimiter/.style={xshift=1ex}}
      \matrix (mat) [matrix of math nodes, left delimiter=(, right delimiter=)] {
\draw[fill=gray] (0,0) rectangle (32,32);
\\
      };
\end{tikzpicture}

==> figure/fig-comp-modules/fig-comp-u1.tex <==
\begin{tikzpicture}[baseline=-0.5ex]
      \tikzset{every left delimiter/.style={xshift=-1ex},every right delimiter/.style={xshift=1ex}}
      \matrix (mat) [matrix of math nodes, left delimiter=(, right delimiter=)] {
\draw;
\foreach \k in {0,2,...,30}{
\foreach \i in {0,0.5,...,1.5} {
    \draw[fill=gray] (32-\i-\k,\k) rectangle (32-\i-\k-0.5,\k+2);
}
}\\
      };
\end{tikzpicture}

==> figure/fig-comp-modules/fig-comp-u2.tex <==
\begin{tikzpicture}[baseline=-0.5ex]
      \tikzset{every left delimiter/.style={xshift=-1ex},every right delimiter/.style={xshift=1ex}}
      \matrix (mat) [matrix of math nodes, left delimiter=(, right delimiter=)] {
\draw;
\foreach \k in {0,1,...,31}{
\foreach \i in {0,0.5} {
    \draw[fill=gray] (32-\i-\k,\k) rectangle (32-\i-\k-0.5,\k+1);
}
}\\
      };
\end{tikzpicture}

==> figure/fig-comp-modules/fig-comp-v1.tex <==
\begin{tikzpicture}[baseline=-0.5ex]
      \tikzset{every left delimiter/.style={xshift=-1ex},every right delimiter/.style={xshift=1ex}}
      \matrix (mat) [matrix of math nodes, left delimiter=(, right delimiter=)] {
\draw;
\foreach \k in {0,2,...,30}{
\foreach \i in {0,0.5,...,1.5} {
    \draw[fill=gray] (\k,32-\i-\k) rectangle (\k+2,32-\i-\k-0.5);
}
}\\
      };
\end{tikzpicture}

==> figure/fig-comp-modules/fig-comp-v2.tex <==
\begin{tikzpicture}[baseline=-0.5ex]
      \tikzset{every left delimiter/.style={xshift=-1ex},every right delimiter/.style={xshift=1ex}}
      \matrix (mat) [matrix of math nodes, left delimiter=(, right delimiter=)] {
\draw;
\foreach \k in {0,1,...,31}{
\foreach \i in {0,0.5} {
    \draw[fill=gray] (\k,32-\i-\k) rectangle (\k+1,32-\i-\k-0.5);
}
}\\
      };
\end{tikzpicture}

==> figure/fig-compression-1D.tex <==
\begin{figure}[htp]
\begin{minipage}{\textwidth}
\centering
\resizebox{3.5cm}{!}{
\input{figure/fig-comp-modules/fig-K}
}
$\approx$
\resizebox{3.5cm}{!}{
\input{figure/fig-comp-modules/fig-uncomp-u}
}
\resizebox{3.5cm}{!}{
\input{figure/fig-comp-modules/fig-M}
}
\resizebox{3.5cm}{!}{
\input{figure/fig-comp-modules/fig-uncomp-v}
}\\
\end{minipage}
\caption{The middle level factorization of
    a $64\times 64$ complementary low-rank matrix $\tilde{M}^h\approx C^3M^3(R^3)^*$
    assuming $r=1$.
    Grey blocks indicate nonzero blocks.
    $C^3$ and $R^3$ are block-diagonal matrices with $8$ blocks.
    The diagonal blocks of $C^3$ and $R^3$ are assembled
    according to Equation \eqref{eq:expression-UV}
    as indicated by black rectangles.
    $M^3$ is a $8\times 8$ block matrix with each block
    $M^3_{i,j}$ itself an $8\times 8$ block matrix
    containing diagonal weights matrix on the $(j,i)$ block.}
\label{fig:compression-1D}
\end{figure}


==> figure/fig-compression-1D2.tex <==
\begin{figure}[htp]
\begin{minipage}{\textwidth}
\centering
\resizebox{3.5cm}{!}{
\input{figure/fig-comp-modules/fig-uncomp-u2}
}
$\approx$
\resizebox{3.5cm}{!}{
\input{figure/fig-comp-modules/fig-uncomp-svd}
}
=
\resizebox{3.5cm}{!}{
\input{figure/fig-comp-modules/fig-comp-u1}
}
\resizebox{3.5cm}{!}{
\input{figure/fig-comp-modules/fig-comp-g1}
}\\
\resizebox{3.5cm}{!}{
}
$\approx$
\resizebox{3.5cm}{!}{
\input{figure/fig-comp-modules/fig-comp-u2}
}
\resizebox{3.5cm}{!}{
\input{figure/fig-comp-modules/fig-comp-g2}
}
\resizebox{3.5cm}{!}{
\input{figure/fig-comp-modules/fig-comp-g1}
}\\
\end{minipage}
\caption{The recursive factorization of $U^3$
    in Figure~\ref{fig:compression-1D}.
    Gray factors are matrices inheriting the complementary low-rank
    property.
    Top: left matrix: $U^3$ with each diagonal block
    partitioned into smaller blocks according to
    Equation \eqref{eqn:half} as indicated by black rectangles;
    middle-left matrix: low-rank approximations of submatrices
    in $U^3$ given by Equation \eqref{eqn:RSh};
    middle right matrix: $U^4$;
    right matrix: $G^3$.
    Bottom: $U^4$ in the first row is further factorized into
    $U^4\approx U^5G^4$, giving $U^3 \approx U^5 G^4 G^3$.}
\label{fig:compression-1D2}
\end{figure}

==> figure/fig-compression-1D3.tex <==
\begin{figure}[htp]
\begin{minipage}{\textwidth}
\centering
\resizebox{3.5cm}{!}{
\input{figure/fig-comp-modules/fig-uncomp-v2}
}
=
\resizebox{3.5cm}{!}{
\input{figure/fig-comp-modules/fig-comp-h1}
}
\resizebox{3.5cm}{!}{
\input{figure/fig-comp-modules/fig-comp-h2}
}
\resizebox{3.5cm}{!}{
\input{figure/fig-comp-modules/fig-comp-v2}
}\\
\end{minipage}
\caption{The recursive factorization $(V^3)^* \approx (H^3)^*(H^4)^*(V^5)^*$ of $(V^3)^*$
    in Figure~\ref{fig:compression-1D}.}
\label{fig:compression-1D3}
\end{figure}


==> figure/fig-domain-tree-BF.tex <==
\begin{figure}
\centering
\begin{tikzpicture}[scale=0.3]

\draw [->,double,double distance=1pt] (-6,5.5) -> (-6,10);

\draw [->,double,double distance=1pt] (-6,4.5) -> (-6,0);

\draw (0,10) -- (-4,0) -- (4,0) -- cycle;

\draw [->,double,double distance=1pt] (20,5.5) -> (20,10);

\draw [->,double,double distance=1pt] (20,4.5) -> (20,0);

\draw (14,10) -- (10,0) -- (18,0) -- cycle;

\draw [latex-latex,line width=1pt] (9,5) -> (5,5);
\draw [latex-latex,line width=1pt] (9,9) -> (5,1);
\draw [latex-latex,line width=1pt] (9,1) -> (5,9);

\coordinate [label=above:$T_X$] (X) at (0,10);
\coordinate [label=above:$T_\Omega$] (X) at (14,10);

\draw (-2,5) -- (2,5);
\draw (12,5) -- (16,5);

\coordinate [label=right:$\frac{L}{2}$] (X) at (16,5);
\coordinate [label=left:$\frac{L}{2}$] (X) at (-2,5);
\end{tikzpicture}
\caption{Trees of the row and column indices.
    Left: $T_X$ for the row indices $X$.
    Right: $T_\Omega$ for the column indices $\Omega$.
    The interaction between $A\in T_X$ and $B\in T_\Omega$
    starts at the middle level of $T_X$ and the leaves of 
    $T_\Omega$ for the middle level factorization. The 
    interaction goes down in $T_X$ and goes up in $T_\Omega$ 
    simultaneously for the recursive factorization of 
    left factors. The interaction goes up in $T_X$ and 
    goes down in $T_\Omega$ 
    simultaneously for the recursive factorization of 
    right factors. }
\label{fig:domain-tree-BF}
\end{figure}

==> figure/fig-double-block-matrix.tex <==
\begin{figure}[htp]
\begin{minipage}{0.32\textwidth}
\begin{tikzpicture}[scale=0.25]
\draw[draw=black] (0,0) rectangle (16,16);
\draw[draw=black,dashed] (0,8) rectangle (16,12);
\draw[draw=black,dashed] (8,0) rectangle (12,16);
\draw[draw=black] (8,8) rectangle (12,12);
\draw[draw=black,dashed] (9,8) rectangle (10,12);
\draw[draw=black,dashed] (8,9) rectangle (12,10);
\filldraw[fill=lightgray,draw=black] (9,9) rectangle (10,10);
\draw (0,10) node[left=3pt,rectangle,fill=white] {$A$};
\draw (10,16) node[above=3pt,rectangle,fill=white] {$B$};
\draw (8,9.5) node[left=3pt,rectangle,fill=white] {{\tiny $C$}};
\draw (9.5,12) node[above=3pt,rectangle,fill=white] {{\tiny $D$}};
\draw (8,0) node[below=5pt,rectangle,fill=white] {$M_{AB,CD}$};
\end{tikzpicture}
\end{minipage}
\caption{The visualization of the submatrices $\{M_{AB,CD}\}$, $\{M_{AB,:D}\}$, and $\{M_{AB,C:}\}$ in $M_{AB}$. The largest black rectangle represents a matrix $M$ and the smaller one inside $M$ indicates its submatrix $M_{AB}$. From left to right, the light gray boxes inside $M_{AB}$ indicate the submatrices  $\{M_{AB,CD}\}$, $\{M_{AB,:D}\}$, and $\{M_{AB,C:}\}$, respectively.}
\label{fig:double-block-matrix}
\end{figure}
